CoCoMo: Computational Consciousness Modeling for Generative and Ethical AI

The CoCoMo model proposes a computational solution to the challenge of incorporating ethical and emotional intelligence considerations into AI systems, with the aim of creating AI agents that combine knowledge with compassion. To achieve this goal, CoCoMo prioritizes fairness, beneficence, non-maleficence, empathy, adaptability, transparency, and critical and exploratory thinking abilities. The model employs consciousness modeling, reinforcement learning, and prompt template formulation to support these desired traits. By incorporating ethical and emotional intelligence considerations, a generative AI model can potentially lead to improved fairness, reduced toxicity, and increased reliability.

==> CaseStudy.tex <==
\section{Case Study: Design a Long-term Care Robot}
\label{sec-case-study}

There are several key challenges facing senior care and long-term care (nursing home care) in the United States and abroad, including issues of affordability, accessibility, quality of care, and even instances of abuse and neglect. Care-giving can also be a physically and emotionally demanding task, and caregivers may not have sufficient support or resources to manage the burden.

\begin{comment}
\begin{figure}[ht!]
%\vspace{-.1in}
\begin{center}
    \centerline{\includegraphics[width=0.99\linewidth]{IMAGES/assistant-living-cost-map.jpeg}}
    %\vspace{-.1in}    
    \caption{US Assistant Living Cost by State, 2022. \\(Source: Genworth. (2022). Cost of Care Survey.)}
    \label{fig:nursinghomecost}
\end{center}
\vspace{-.2in}
\end{figure}
\end{comment}

In order to address these challenges and improve the quality of care for seniors, we plan to develop an artificial agent that could assist with various day-to-day caring tasks. 
The design process follows these steps:

\begin{noindlist}
    \item Identifying key requirements for a healthcare artificial agent.
    \item Conducting a feasibility assessment on the top five requirements on the list.
    \item Identifying three requirements that could potentially be addressed by existing system-1 AI capabilities, and explaining how these could be implemented.
    \item Selecting one ``hard'' requirement to tackle through the development of system-2 AI capabilities.
    \item Sketching out our design and technical tasks, and working towards implementation.
    \item Making the design adaptive to personal needs and preferences.
\end{noindlist}

At the top level, we would like an AI agent to help a care recipient become a better version of themselves day by day. This can be achieved through improving various aspects of the care recipient's life, such as their health, happiness, and sense of beauty. These goals can be communicated to the AI agent through prompting templates that provide positive and negative examples. Improving the effectiveness of these templates is a critical research area for this case study.

To meet these goals, the AI agent should have certain functional capabilities, including the ability to perform preliminary diagnosis on the care recipient's health condition, access a knowledge base of relevant diseases and conditions, and display desired attributes such as attentiveness, empathy, patience, love, and humor. Any health concerns identified by the AI agent should be escalated to human supervisors through defined protocols.

To fulfil this list of requirements, we consider that
using SCM with medical IoTs as extended signal receptors is sufficient
to form a hardware baseline. Regarding medical
domain knowledge and disease diagnosis and prediction,
various vital-signing monitoring, diagnostic
algorithms, and remedy recommendations
have been developed and are ready to interoperate. 
Please consult an extended survey including our
own healthcare documented in \cite{ChangTricorder2022}.  


==> EmpiricalConfirmation.tex <==
\subsection{Empirical Confirmation}
\label{sec-where}

We now tie the theoretical models presented in
the previous section with the physical
brain and the central nervous system (CNS).


Conscious thoughts are processed by the brain. Specifically, the prefrontal cortex, which is the part of the brain responsible for higher cognitive functions such as decision making, problem solving, and planning, is thought to play a key role in the processing of conscious thoughts. The prefrontal cortex is also thought to be involved in the integration of information from various other brain regions, allowing us to make sense of the thoughts and experiences that we have. Other brain regions that are important for the processing of conscious thoughts include the parietal lobe, which is involved in the integration of sensory information, and the temporal lobe, which is important for the processing of language and memory.

One approach to understanding the neural basis of consciousness is to identify the specific brain regions or processes that are necessary for conscious experience. For example, research has suggested that the prefrontal cortex, the thalamus, and the reticular activating system may play a role in conscious processing. However, it is important to note that these brain areas are not the sole source of consciousness, and that many other brain regions and processes likely also contribute to conscious experience.

Other factors that may contribute to consciousness include the activity of neurotransmitters such as dopamine and serotonin, as well as the presence of certain brain waves. Some researchers have also suggested that consciousness may involve the interaction of multiple brain systems, including those involved in perception, attention, and memory.


Another approach to understanding the neural basis of consciousness is to consider how different brain areas and processes work together to support conscious experience. For example, the global workspace theory proposes that conscious experience arises from the integration of information from different brain regions through interactions in the prefrontal cortex.

To verify these theories, 
Stanislas Dehaene and Jean-Pierre Changeux in~\cite{dehaene2011experimental} reviewed and discussed a range of experimental studies on the neural basis of conscious processing, including neuroimaging, neurophysiological, and lesion, and transcranial magnetic stimulation studies.
More specifically, the experimental studies discussed in the article include:

\begin{itemize}
\item 
Neuroimaging studies using functional magnetic resonance imaging (fMRI) and positron emission tomography (PET) to investigate the brain areas and processes involved in conscious processing \cite{dehaene2001imaging,dehaene2006conscious}.
\item 
Neurophysiological studies using electrophysiological techniques, such as electroencephalography (EEG) and magnetoencephalography (MEG), to study the brain activity associated with conscious processing \cite{dehaene2003neural,dehaene2011experience}.
\item
Lesion studies, which involve examining the effects of brain damage on conscious processing, to identify the brain areas and processes necessary for conscious experience~\cite{binetti1998cortical,dehaene1998cerebral}.
\item
Studies using transcranial magnetic stimulation (TMS) to manipulate brain activity and investigate the causal role of specific brain areas in conscious processing~\cite{koch2006magnetic,massimini2005breakdown}.
\item
Studies using single-neuron recording techniques in non-human primates to investigate the neural basis of conscious perception and decision-making~\cite{lau2006dissociable,quianquiroga2005invariant}.
\item
Studies using pharmacological manipulations to investigate the role of specific neurotransmitter systems in 
conscious processing~\cite{dehaene2006conscious}.
\end{itemize}

The experimental studies discussed in the article provide insights into the neural basis of conscious processing and how different brain systems and processes contribute to conscious experience.
The authors propose a framework for understanding the neural basis of conscious processing, which involves three levels of analysis: the {\em neuronal} level, the {\em network} level, and the {\em global} level.
At the neuronal level, the authors discuss the role of various brain areas, including the prefrontal cortex and the thalamus, in conscious processing. They also discuss the importance of neurotransmitters and oscillations in the brain in supporting conscious processing.
At the network level, the authors discuss how different brain areas work together to support conscious processing, and how this involves the integration of information from multiple brain systems.
At the global level, the authors discuss how conscious processing depends on the integration of information from multiple sources and how this integration is supported by the prefrontal cortex. They also discuss how this integration allows for the emergence of higher-level cognitive functions, such as attention and decision-making.

Overall, the article provides an overview of how different brain processes and systems contribute to conscious processing, and how this understanding can be used to develop computational models of consciousness.

\begin{comment}
\subsection{Consciousness and Unconsciousness Transitions}

There are several theories about the mechanisms underlying the transition from unconsciousness to consciousness. We have mentioned that GWT considers
that the prefrontal cortex acts as a central hub for integrating and processing information from various sensory and cognitive systems. When an event or stimulus is perceived as important or novel, it is thought to be broadcast to the prefrontal cortex and other brain regions for further processing and action. This process is thought to give rise from unconscious to conscious experience with respect to the event. Similarly, The IIT theory suggests that consciousness arises from the integration of information across multiple brain systems. According to this theory, the transition from unconsciousness to consciousness involves the integration of information in a way that is both rich and differentiated.

Erwin Schrödinger, a famous physicist, put the theories and empirical evidences
into a quantifiable framework that computers can execute. 
Schrödinger discussed the concept of the transition from unconsciousness to consciousness in his book "What is Life?". Schrödinger proposed that the second law of thermodynamics, which states that entropy (a measure of disorder or randomness) in a closed system will always increase over time, could be used to understand the transition from consciousness to unconsciousness. He suggested that this transition occurs when there is an increase in the randomness or disorder of matter, such as when a task becomes habitual and the brain enters an inert state.

In addition to the second law of thermodynamics, Schrödinger also proposed that quantum mechanical processes, such as quantum jumps or superpositions, may play a role in the transitions between unconsciousness and consciousness. He suggested that these processes may be triggered when the accumulated energy in a neural region reaches a threshold. When this happens, the region of the brain responsible for managing consciousness is alerted to pay attention to the emergent event and to plan for reactions.

Overall, while the exact mechanisms underlying the transition from unconsciousness to consciousness are not fully understood, the global workspace theory and the integrated information theory provide important insights into this process. Schrödinger's ideas also suggest that the second law of thermodynamics and quantum mechanical processes may be involved in these transitions.

\end{comment}

==> IEEENotes.tex <==
\subsection{Some Common Mistakes}\label{SCM}
\begin{itemize}
    \item The word ``data'' is plural, not singular.
    \item The subscript for the permeability of vacuum $\mu_{0}$, and other common scientific constants, is zero with subscript formatting, not a lowercase letter ``o''.
    \item In American English, commas, semicolons, periods, question and exclamation marks are located within quotation marks only when a complete thought or name is cited, such as a title or full quotation. When quotation marks are used, instead of a bold or italic typeface, to highlight a word or phrase, punctuation should appear outside of the quotation marks. A parenthetical phrase or statement at the end of a sentence is punctuated outside of the closing parenthesis (like this). (A parenthetical sentence is punctuated within the parentheses.)
    \item A graph within a graph is an ``inset'', not an ``insert''. The word alternatively is preferred to the word ``alternately'' (unless you really mean something that alternates).
    \item Do not use the word ``essentially'' to mean ``approximately'' or ``effectively''.
    \item In your paper title, if the words ``that uses'' can accurately replace the word ``using'', capitalize the ``u''; if not, keep using lower-cased.
    \item Be aware of the different meanings of the homophones ``affect'' and ``effect'', ``complement'' and ``compliment'', ``discreet'' and ``discrete'', ``principal'' and ``principle''.
    \item Do not confuse ``imply'' and ``infer''.
    \item The prefix ``non'' is not a word; it should be joined to the word it modifies, usually without a hyphen.
    \item There is no period after the ``et'' in the Latin abbreviation ``et al.''.
    \item The abbreviation ``i.e.'' means ``that is'', and the abbreviation ``e.g.'' means ``for example''.
\end{itemize}


\subsection{Authors and Affiliations}
\textbf{The class file is designed for, but not limited to, six authors.} A
minimum of one author is required for all conference articles. Author names
should be listed starting from left to right and then moving down to the
next line. This is the author sequence that will be used in future citations
and by indexing services. Names should not be listed in columns nor group by
affiliation. Please keep your affiliations as succinct as possible (for
example, do not differentiate among departments of the same organization).

\subsection{Identify the Headings}
Headings, or heads, are organizational devices that guide the reader through
your paper. There are two types: component heads and text heads.

Component heads identify the different components of your paper and are not
topically subordinate to each other. Examples include Acknowledgments and
References and, for these, the correct style to use is ``Heading 5''. Use
``figure caption'' for your Figure captions, and ``table head'' for your
table title. Run-in heads, such as ``Abstract'', will require you to apply a
style (in this case, italic) in addition to the style provided by the drop
down menu to differentiate the head from the text.

Text heads organize the topics on a relational, hierarchical basis. For
example, the paper title is the primary text head because all subsequent
material relates and elaborates on this one topic. If there are two or more
sub-topics, the next level head (uppercase Roman numerals) should be used
and, conversely, if there are not at least two sub-topics, then no subheads
should be introduced.

\subsection{Figures and Tables}
\paragraph{Positioning Figures and Tables} Place figures and tables at the top and
bottom of columns. Avoid placing them in the middle of columns. Large
figures and tables may span across both columns. Figure captions should be
below the figures; table heads should appear above the tables. Insert
figures and tables after they are cited in the text. Use the abbreviation
``Fig.~\ref{fig}'', even at the beginning of a sentence.

\begin{table}[htbp]
    \caption{Table Type Styles}
    \begin{center}
        \begin{tabular}{|c|c|c|c|}
            \hline
            \textbf{Table} & \multicolumn{3}{|c|}{\textbf{Table Column Head}}                                                         \\
            \cline{2-4}
            \textbf{Head}  & \textbf{\textit{Table column subhead}}           & \textbf{\textit{Subhead}} & \textbf{\textit{Subhead}} \\
            \hline
            copy           & More table copy$^{\mathrm{a}}$                   &                           &                           \\
            \hline
            \multicolumn{4}{l}{$^{\mathrm{a}}$Sample of a Table footnote.}
        \end{tabular}
        \label{tab1}
    \end{center}
\end{table}

\begin{figure}[htbp]
    \centerline{\includegraphics{fig1.png}}
    \caption{Example of a figure caption.}
    \label{fig}
\end{figure}

Figure Labels: Use 8 point Times New Roman for Figure labels. Use words
rather than symbols or abbreviations when writing Figure axis labels to
avoid confusing the reader. As an example, write the quantity
``Magnetization'', or ``Magnetization, M'', not just ``M''. If including
units in the label, present them within parentheses. Do not label axes only
with units. In the example, write ``Magnetization (A/m)'' or ``Magnetization
\{A[m(1)]\}'', not just ``A/m''. Do not label axes with a ratio of
quantities and units. For example, write ``Temperature (K)'', not
``Temperature/K''.


==> Introduction.tex <==
\section{Introduction}
\label{sec:intro}

Narrow AI, also known as system-1 AI \cite{kahneman2011thinking}, is designed for performing specific, predefined tasks using machine learning algorithms, such as object recognition and language translation. However, when it comes to more complex generative AI tasks such as reasoning, critical and exploratory thinking, and emotion and behavior modeling and regulation, system-1 AI falls short.

To address these limitations, researchers (e.g., Yoshua Bengio \cite{bengio2020future}) have proposed the development of system-2 AI, which aims to mimic human cognitive abilities. Several generative models have been developed since 2022 for text \cite{brown2020language, LAMDA2022, chatgpt}, image \cite{LatentDiffusionModels, DALL-E2022}, and video generation \cite{VideoMeta2022}. However, these models face issues of bias, toxicity, robustness, and reliability \cite{RisksLLM2022, AIEthicsChatGPT2023}.

In this paper, we propose a solution to address these concerns by modeling emotional intelligence and ethical guardrails within a generative AI model itself, drawing on insights from the study of human consciousness. We believe that addressing these issues outside of a generative AI model is equivalent to imposing censorship on user-generated content, which is a difficult and non-scalable task \cite{SocialMediaMisInfo2021,SiliconValues}.

Human consciousness is believed to regulate impulsive and reflective unconsciousness to make compromises between competing goals and values. Understanding how human consciousness works, both physically and functionally, can help us gain valuable insights for developing a regulator that guides behavior and creativity in a generative AI model.

The nature and origin of consciousness have been studied for centuries, resulting in various theories, including the global workspace theory \cite{baars1988cognitive}, integrated information theory \cite{tononi2004information, tononi2008consciousness, tononi2016phi}, neural correlates of consciousness approach \cite{koch2004quest, crick1990towards}, and attention schema theory \cite{graziano2013consciousness, graziano2016attention}, among others. These studies of consciousness provide valuable insights for architecting system-2 AI.

Drawing on the functionalist approach\footnote{Functionalism proposes that consciousness arises from the function of the brain, rather than its specific physical or neural implementation \cite{putnam1967psychological,fodor1968functional}. Section~\ref{sec-panpsychism-functionalism} provides
justifications.} to model consciousness, 
this paper defines the desired traits and capabilities of system-2 AI, which include knowledge, fairness, beneficence, non-maleficence, empathy, adaptability, transparency, and critical and exploratory thinking abilities. While this list is not exhaustive, it provides a starting point for developing ethical guardrails and emotional intelligence in AI systems. Depending on the context and application of AI, additional ethical considerations or modifications to these principles may be necessary.

To embody these capabilities and principles, we introduce the Computational Consciousness Model (CoCoMo), which leverages priority-based scheduling, reward-based optimization, and Socratic dialogues. CoCoMo offers customization based on cultural and individual requirements through adaptive prompt templates \cite{PromptSurvey2023, SocraticIEEECCWC2023}, and facilitates the transition between unconsciousness and consciousness states through a multi-level feedback scheduler and interrupt mechanism. To enable emotion and behavior modeling and regulation, and critical and exploratory thinking, CoCoMo interacts with large language models \cite{OpenAI-GPT3-2020, LAMDA2022, chatgpt, BioGPT2022} using interactive question-answer-based dialogues. Furthermore, a reinforcement learning module maps external values and rewards that it learns to internal task-scheduling priorities. CoCoMo has the potential to support adaptive computational consciousness that integrates knowledge with compassion.

In conclusion, we believe that CoCoMo has the potential to model and enhance emotional intelligence for generative AI systems, benefiting humanity and society. The paper is structured into several sections, including a survey of related work in various fields to define consciousness for computational modeling in Section~\ref{sec-what-survey}, a list of System-2 AI capabilities in Section~\ref{sec-goals}, a proposal of CoCoMo, its modules, functions, and algorithms in Section~\ref{sec-CoCoMo}, and concluding remarks and open issues for future research in Section~\ref{sec-conclusion}.

\begin{comment}
Overall, the paper proposes a novel approach to addressing the challenges of generative AI systems. By modeling emotional intelligence and ethical values in a generative AI model itself, we can develop guardrails to mitigate issues such as bias and toxicity and improve the performance of the model in terms of robustness and reliability. The proposed Computational Consciousness Model is a promising direction for future research in this area.
\end{comment}


==> Models.tex <==

Panpsychism is a broad and abstract philosophical theory that proposes that consciousness is a fundamental aspect of the universe and is present in all matter. While panpsychism has inspired a number of more specific models or theories developed by neuroscientists and psychiatrists, one of the most well-known is the integrated information theory (IIT) proposed by Giulio Tononi.

According to the IIT, consciousness arises from the integration of information within a system, and can be quantified using a measure called phi. Tononi and his colleagues have proposed that phi can be used to distinguish between conscious and unconscious states, and that it is a fundamental property of the universe.

Another well-known model of panpsychism is the global workspace theory (GWT), proposed by Bernard Baars. The GWT suggests that consciousness arises from the global activation of neurons in the brain, which allows for the integration of information from multiple sources and the creation of a unified conscious experience.

The neural correlates of consciousness (NCC) approach, proposed by Francis Crick and Christof Koch, suggests that consciousness arises from the activity of specific neural networks in the brain. According to this approach, identifying the neural correlates of consciousness can help us understand the mechanisms underlying conscious experience.

Finally, the attention schema theory (AST) proposed by Michael Graziano suggests that consciousness arises from the brain's ability to model its own attentional processes. According to the AST, the brain constructs a simplified model of attention, which is then used to explain conscious experience.

Overall, these and other models and theories of panpsychism seek to provide more detailed or nuanced explanations for the nature of consciousness, and to explore the implications of panpsychism for our understanding of the mind and the physical world.





==> RelatedWork.tex <==
\section{Related Work}

Artificial consciousness is a field of study that aims to understand and create conscious-like states in artificial systems, such as computers and robots. Researchers in this field aim to understand the fundamental nature of consciousness and how it might be artificially reproduced.

There are many different theories and approaches to artificial consciousness, including:

Functionalism: This approach proposes that consciousness can be understood as a mental or computational process that performs certain cognitive functions, such as perception, attention, and decision-making. According to functionalism, consciousness does not depend on specific physical or neural implementation, but rather on the functions it performs.

Panpsychism: This approach proposes that consciousness is a fundamental property of the universe and that all physical entities, including inanimate objects, have some form of consciousness.

Neuromorphic engineering: This approach seeks to create artificial systems that mimic the structure and function of the brain in order to create conscious-like states.

In this article, we survey these theories in depth and present
our thoughts to model and implement artificial consciousness for specific 
aims and constraints. 

==> Stale-Comp-Model-Long.tex <==
subsection{Review of Theoretical Models}

Let us first discuss representative theoretical
models developed by psychiatrists and neuroscientists. 
Their designs are founded on brain study and behavior study, rather than just some philosophical
thoughts. These models attempt to explain how consciousness arises from the 
activity of the brain, and how it might be simulated 
in artificial systems such as computers.

\hfill \break
\noindent{\bf Global Workspace Theory} (GWT):
GWT was proposed by Bernard Baars in 1988 \cite{baars1988cognitive}.  GWT is
also known as the {\em global neuronal workspace} (GNW).
Baars' contributions to the development of the GNW theory include the following:

\begin{enumerate}
\item 
He developed the original conceptual framework for the GNW theory, which proposes that consciousness arises from the integration of information from multiple brain systems through interactions in the prefrontal cortex.
\item
He proposed the idea that the prefrontal cortex acts as a central hub that integrates information from various brain systems and broadcasts this information to other brain regions, a key aspect of the GNW theory.
\item
He developed a computational model of the GNW theory, which specifies the algorithms and processes that underlie the integration of information in the prefrontal cortex.
\item
He provided empirical evidence for the GNW theory through a series of experimental studies, which have been influential in shaping our understanding of the neural basis of consciousness.
\end{enumerate}

%(Four keywords of GWT are sensing, information, attention, integration, and memory.)
 
\hfill \break
\noindent{\bf Integrated Information Theory} (IIT):
According to IIT, proposed by Giulio Tononi \cite{tononi2004information}, consciousness arises from the integration of information across multiple sources and is characterized by the ability to distinguish between different states of the system. IIT proposes that the amount of consciousness in a system can be quantified by a measure called $\phi$, which reflects the degree of integration of information in the system. For example, consider a simple system with two parts, A and B. If the state of A does not affect the state of B, and the state of B does not affect the state of A, then there is no integration of information between the two parts, and the system has zero $\phi$. On the other hand, if the state of A does affect the state of B, and the state of B does affect the state of A, then there is integration of information between the two parts, and the system has non-zero $\phi$ value.
%(Two keywords of IIT are information and integration.)

\hfill \break
\noindent{\bf Dynamic Core Hypothesis} (DCH):
DCH was developed by neuroscientist Bernard Edelman \cite{edelman2000dynamic}. DCH proposes that consciousness arises from the activity of a specialized region of the brain called the thalamocortical system, which is made up of the thalamus and the cortex. According to the theory, the thalamocortical system is a dynamic network of neurons that constantly adjusts its activity in response to sensory input, motor output, and other internal and external influences. This dynamic activity is thought to give rise to the subjective experience of consciousness.

One key aspect of the Dynamic Core Hypothesis is the idea that consciousness is not a unitary, all-or-none phenomenon, but rather a continuous, graded property of the brain. According to the theory, different brain states can give rise to different levels of consciousness, depending on the degree of integration and differentiation of activity in the thalamocortical system. For example, a person who is deeply asleep or under general anesthesia would have a low level of consciousness, while a person who is fully awake and alert would have a high level of consciousness.

The Dynamic Core Hypothesis also proposes that consciousness is closely tied to the brain's ability to generate predictions about the environment and to update those predictions based on new information. This predictive coding process is thought to be mediated by the thalamocortical system, and it is thought to be essential for the experience of consciousness. 

%(Five keywords of DCH are information, integration, level/degree, prediction, and update.)

\hfill \break
\noindent{\bf Attention Schema Theory} (AST):
AST is a theory of consciousness developed by neuroscientist Michael Graziano \cite{graziano2013attention,graziano2016attention}. AST proposes that consciousness arises from the brain's representation of attention as a computational process. According to the theory, the brain constructs a model or schema of attention that it uses to represent the attention states of both itself and others. 
The attention schema for itself creates a sense of self and a subjective 
experience of attention. 
(This attention schema is thought to be a way of representing the concept of attention in the brain, rather than being a direct representation of attention itself.)

According to AST, the attention schema is constructed by the brain in order to facilitate communication and social interaction. It allows the brain to predict and interpret the attention states of others, which is important for understanding their intentions and behaviors. The attention schema is also thought to play a role in the brain's ability to allocate its own attention resources, allowing it to focus on relevant stimuli and ignore distractions.

%(Five keywords are attention, schema, subjectivity, communication and prediction.)

